PINT: Probabilistic In-band Network Telemetry

Commodity network devices support adding in-band telemetry measurements into data packets, enabling a wide range of applications, including network troubleshooting, congestion control, and path tracing. However, including such information on packets adds significant overhead that impacts both flow completion times and application-level performance. We introduce PINT, an in-band telemetry framework that bounds the amount of information added to each packet. PINT encodes the requested data on multiple packets, allowing per-packet overhead limits that can be as low as one bit. We analyze PINT and prove performance bounds, including cases when multiple queries are running simultaneously. PINT is implemented in P4 and can be deployed on network devices. Using real topologies and traffic characteristics, we show that PINT concurrently enables applications such as congestion control, path tracing, and computing tail latencies, using only sixteen bits per packet, with performance comparable to the state of the art.

==> Analysis.tex <==
\section{Full Analysis}\label{app:analysis}
%Our analysis leverages known techniques for the Poissonization of a Balls-and-Bin stochastic process~\cite{?}.
%\ran{Anything below this point would go to a full version?}

The following bounds the number of samples we need from  some distance $d\in\set{1,\ldots,k}$ in order to successfully recover the $d$'th switch on the path with probability $1-\delta/k$.
%[*** I think these examples should come AFTER the theorems;  you don't have the expressions in front of you when you see the examples***]
\begin{theorem}
Let $Z=\ceil{-\frac{\log_2 (1-(1-\delta/k)^{1/|V|})}{\mathfrak b}}$ and $d\in\set{1,\ldots,k}$; after seeing $Z$ packets from distance $d$, $$\Pr[|V_d|>1]<\delta/k.$$
\end{theorem}
\begin{proof}
Consider all switches are are not the $d$'th switch on the path. Each such switch has a probability of $2^{-\mathfrak b}$ of agreeing with each sample. 
Therefore, fixing each switch in $|V|$, the number of samples we require until it disagrees with at least one sample is geometrically distributed with parameter $1-2^{-\mathfrak b}$.
Our goal is therefore to bound $\max_{i\le |V|} X_i$ for i.i.d. random variables $X_i\sim\mbox{Geo}(1-2^{-\mathfrak b})$.
To that end, notice that
\begin{multline*}
    \Pr[\max_{i\le |V|} X_i > Z] = 1-\Pr[\forall {i\le |V|}: X_i \le Z]
    \\=1-(\Pr[X_i \le Z])^{|V|}
    =1-\parentheses{1-(\Pr[X_i > Z])}^{|V|}
    \\= 1-\parentheses{1-(2^{-\mathfrak b})^{ Z}}^{|V|}\le\delta/k.\qedhere
\end{multline*}
%Let $Z=\ceil{-\frac{\log_2 (1-(1-\delta)^{1/|V|})}{b}}$. Then:
%\begin{multline*}
%1-\parentheses{1-(2^{-\mathfrak b})^Z}^{|V|}
%=1-\parentheses{1-(2^{-\mathfrak b})^Z}^{|V|}
%\end{multline*}
%Therefore, the number of samples needed to eliminate all wrong switches is a Negative Binomial random variable with parameters $|V|-1,1-2^{-\mathfrak b}$.
\end{proof}
We can then use the union bound over all distances $d\in\set{1,\ldots,k}$ to conclude the following. For example, if $|V|=100, k=10, \delta=2\%$ and $\mathfrak b=16$, we only require one such sample. If we only have $\mathfrak b=1$ bits per packet, we would require $Z=15$ samples from each distance.
\begin{corollary}
After collecting $Z$ samples from each distance, \sys is able to successfully decode the entire path with probability $1-\delta$.
\end{corollary}
Next, we proceed with proving a bound on $N$ -- the number of distinct slots our algorithm needs to see before it collects $Z$ samples from each distance.
This problem is known as the Double Dixie Cup problem~\cite{DoubleDixie}, which is a generalization of the well studied Coupon Collector problem. 
To interpret the result, observe that $Z < \ceil{\log_2(k|V|/\delta)/\mathfrak b}$ and thus $N = O (k \cdot (\log(k/\delta)+\log(|V|)/\mathfrak b))$. As an example, if $k=10, |V|=100, \delta=5\%$ and $\mathfrak b = 16$, we have $Z=1$ and $N=116$. 
\begin{theorem}\label{thm:NVal}
%Let $C_{m,n}$ be the number of coupons a collector needs to buy before completing $m$ copies of the $n$-coupons collection. Then
After seeing {\small $$N=\NVal$$}
distinct slots, our algorithm has at least $Z$ samples from each distance and is able to reconstruct the path successfully.
\end{theorem}
\begin{proof}
%[*** Siunce we used $X_i$ in the last theorem, we might at least consider if we should use a different variable, but it reads OK. ***]
Our algorithm uses Reservoir Sampling to sample each distance with the same probability. Therefore, the number of samples of distance $i$ are a binomial random variable we denote by $Y_i\sim \mathit{Bin}(N,1/k)$.
Our goal is to show that getting $Y_i< Z$ is unlikely; to that end, we use the Chernoff inequality that states that $\Pr[Y_i\le \mathbb E[Y_i](1-\gamma)]\le e^{-\mathbb E[Y_i]\gamma^2/2}$ for any $\gamma\in(0,1]$. We set $\gamma=1-k(Z-1)/N$ to get
\begin{multline*}
    \Pr[Y_i< Z] = \Pr[Y_i\le Z-1] = \Pr[Y_i\le \mathbb E[Y_i](1-\gamma)]
    \\ \le e^{-\mathbb E[Y_i]\gamma^2/2} 
    = e^{-N/2k\cdot (1-k(Z-1)/N)^2}
    \\= e^{-(N/2k -(Z-1)+k(Z-1)^2/2N)}
    = e^{-(x -(Z-1)+(Z-1)^2/4x)},
\end{multline*}
where $x=N/(2k)$. We want $\Pr[X_i< Z]\le \delta/k$, which according to the above follows from
\begin{multline*}
    x -(Z-1)+(Z-1)^2/4x\ge \ln k/\delta \iff\\
     \mbox{\small $x\ge \xVal$.}
\end{multline*}
The last inequality follows directly from our choice of $N$. Finally, we use the union bound to get that after $N$ samples all distances get at least $Z$ samples except with probability $k\cdot \Pr[Y_i< Z]\le \delta$.
\end{proof}

We proceed with the last part of the main algorithm analysis -- bounding the number of packets needed for getting $N$ distinct slots.
Intuitively, the above analysis provides a quantity $N$ (that depends on $|V|,k,\mathfrak b$, and $\delta$) such that we identify the path after seeing $N$ distinct slots. Recall that $f$ is a random mapping from packet identifiers to the range $\{1,\ldots,r\}$. 
If we set $r=2N$ then, in expectation, we will not require
%more than 
$1+1/(1-1/r)+\ldots+1/(1-(N-1)/r)= r(H_r-H_{r-N})\approx N\cdot 2\ln2\approx 1.39N$  packet to get $N$ distinct slots and identify the path. Here, $H_i\approx \ln i$ is the $i$'th harmonic number.
We now show that we get can a high-probability bound which ensures that the actual number of packets will be close to this expectation.
In our proof, we use the following fact.
\begin{fact}\label{fact}
For any positive real number
$\epsilon\in\mathbb R^+$, 
$$1+\epsilon+\sqrt{2\epsilon}-\ln(1+\epsilon+\sqrt{2\epsilon})\ge 1+\epsilon.$$
\end{fact}
Our proof also makes use of the following theorem, proven in~\cite{janson2018tail}. Intuitively, the time until we see the $i$'th distinct $f$-value is distributed geometrically with parameter $1/(1-(i-1)/r)$ and we wish to bound $A=\sum_{i=1}^N A_i$ which satisfies $\mathbb E[A] = \sum_{i=1}^N \mathbb E[A_i] = r(H_r-H_{r-N})\approx r\log\parentheses{r/(r-N)}$.
\begin{theorem}\label{thm:geoSum}(\cite{janson2018tail})
Let $\{A_1,\ldots A_N\}$ be independent geometric random variables such that $A_i\sim Geo(p_i)$ and $p_1\ge\ldots\ge p_N$. Then the sum $A=\sum_{i=1}^N A_i$ satisfies:
$$
\Pr\brackets{A > \mathbb E[A]\cdot \lambda}\le e^{-p_N\mathbb E[A](\lambda-1-\ln\lambda)}.
$$
\end{theorem}
We are now ready to prove the main theorem which shows the correctness of our algorithm.
\begin{theorem}\label{thm:partialCouponCollector}
Let $\mathbb E[A]= r(H_r-H_{r-N})$ denote the expected number of packets required for seeing $N$ distinct slots.
With probability $1-\delta$, the number of packets our algorithm requires for seeing at least $N$ distinct slots is at most
$$
{\mathbb E[A]+\frac{r\ln\delta^{-1}}{(r-N)}+\sqrt{\frac{2r\mathbb E[A]\ln\delta^{-1}}{(r-N)}}}.
$$
\end{theorem}
\begin{proof}
We wish to use Theorem~\ref{thm:geoSum}; notice that 
we need $\lambda-\ln\lambda\ge 1+\frac{\ln\delta^{-1}}{p_N\mathbb E[A]}$ which implies
$$
e^{-p_N\mathbb E[A](\lambda-1-\ln\lambda)}\le \delta.
$$
According to Fact~\ref{fact}, for $\epsilon=\frac{\ln\delta^{-1}}{p_N\mathbb E[A]}$, it is enough to set 
$$\lambda = 1+\frac{\ln\delta^{-1}}{p_N\mathbb E[A]}+\sqrt{\frac{2\ln\delta^{-1}}{p_N\mathbb E[A]}}.$$
Plugging in $p_N=(1-(N-1)/r) > (r-N)/r$
%and $E[A]=r(H_r-H_{r-N})$ 
we have that the required number of required packets is at most
\begin{multline*}
\lambda\cdot \mathbb E[A] = \parentheses{\mathbb E[A]+\frac{\ln\delta^{-1}}{p_N}+\sqrt{\frac{2\mathbb E[A]\ln\delta^{-1}}{p_N}}}\\
\le \parentheses{\mathbb E[A]+\frac{r\ln\delta^{-1}}{(r-N)}+\sqrt{\frac{2r\mathbb E[A]\ln\delta^{-1}}{(r-N)}}}
.
\end{multline*}
For example, if $r=2N$, we have $\mathbb E[A]\approx 1.39 N$ and the number of packets is 
\begin{multline*}
\parentheses{\mathbb E[A]+{2\ln\delta^{-1}}+\sqrt{{4\mathbb E[A]\ln\delta^{-1}}}}\\\approx
\parentheses{1.39 N+{2\ln\delta^{-1}}+2.35\sqrt{N\ln\delta^{-1}}}
.\qedhere
\end{multline*}
\end{proof}
To illustrate the meaning of this result, recall that our algorithm needed $N=116$ packets to identify the path expect with $5\%$ error probability. This means that the constant-per-packet work algorithm would require $$\parentheses{1.39 N+{2\ln 20}+2.35\sqrt{N\ln 20}}\approx 211$$ packets to find the path, except with probability $10\%$. We note that, as illustrate by our evaluation, this quantity is a loose upper bound and our algorithm is likely to reconstruct the path even with significantly fewer packets.
We now with conclude the number of packets altogether for a successful detection of a $k$-hops path. 
\begin{corollary}
The number of hashes required by our algorithm for a successful identification of a $k$-hops path is
\begin{multline*}
r(H_r-H_{r-N})
+{2\ln2\delta^{-1}}+\sqrt{{4r(H_r-H_{r-N})\ln2\delta^{-1}}}
,
%\\\approx N\cdot r\ln(r/(r-N))+{2\ln\delta^{-1}}+\sqrt{{4N\cdot r\ln(r/(r-N))\ln\delta^{-1}}}
\end{multline*}
where 
$N$ is the number of distinct slots required as specified in Theorem~\ref{thm:NVal}.
\end{corollary}
\renewcommand{\arraystretch}{1.3}
\begin{table*}[]
\begin{center}
\begin{tabular}{c|l}
\hline
\textbf{Use Case} 		& \textbf{Description} 	\\ \hline
\hline
Flow path 		& The path taken by a given flow				\\ \hline
Flowlet path      	& The path taken by a subset of packets belonging to a flow	\\ \hline
DDoS sources      	& Get statistics of DDoS attack sources                      	\\ \hline
Load imbalance      	& Get fine-grained statistics of all flows on a set of links    \\ \hline
Loop freedom		& Detect forwarding loops					\\ \hline
Routing misconfiguration& Identify unwanted path taken by a given flow			\\ \hline
Waypoint Routing	& Identify packets not passing through a waypoint 		\\ \hline
Max Path Length		& No packet should exceed path length of size \textit{n}	\\ \hline
Traffic Matrix		& Get traffic volume between switch pairs			\\ \hline
Congested link diagnosis& Find flows using a congested link, to help rerouting		\\ \hline
Active connections	& Find the number of flow using a given path			\\ \hline
Path conformance	& Checks for policy violations of the path taken by a given flow\\ \hline
\end{tabular}
\end{center}
\caption{Use Cases}
\label{tab:use-cases}
\end{table*}

Next, we analyze our loop-detection extension. We first show a bound on the probability of a false loop reporting. Assume that the packet traverses through a $k$-hop path (without a loop).
Observe that, in Algorithm~\ref{alg:loop}, we only report a loop once $c=T$ and another switch $s$ for which $p_j.\mbox{dig} = h(s,f(p_j))$ sees the packet. This means that the number of switches that has the same hash value on the path is \emph{at least} $T+2$. 
%We consider two cases; first, the probability of having a collision of $T+3$ or more switches can simply be bounded by ${k\choose T+3}\cdot 2^{-\mathfrak b\cdot (T+2)}$. Next, we analyze the $(T+2)$-collisions case more carefully. 
We union bound over all combination of $T+2$ switches on the path that may have caused the false report.
Observe that, given that there are $(T+2)$ such collisions, this will result in a false loop reporting only if (1) the first colliding switch samples the packet and writes its hash, and (2) no switch between the first and second colliding switches samples the packet. Denoting the hop number of the first switch by $a$ and that of the second switch by $q$, the probability of (1) is $1/a$ and the probability of (2) is $a/(q-1)$, and the two are independent. Therefore, the probability of the false report, in this case, is $1/a\cdot a/(q-1) = 1/(q-1)$. Next, we analyze the chance of such collision. There are $q-1$ possible locations for the first colliding switch and ${k-q \choose T}$ options for the locations of the remaining $T$ colliding switches. We conclude the following.
\begin{theorem}
The probability of reporting a false loop in \sys is at most 
$$
2^{-\mathfrak b\cdot (T+1)}\cdot
%\parentheses{{k\choose T+3}2^{-\mathfrak b}+
\sum_{q=2}^{k-T}{k-q \choose T}.
$$
\end{theorem}
For example, when $T=3, k\le10$ and $\mathfrak b=14$ we have that the probability of a false positive is at most $4.4\cdot10^{-13}$.


Finally, we consider the false negative probability. Intuitively, our algorithm would never miss a loop if it were not for the mechanism which drops packets whose TTL have zeroed.
Yet, we can show that if the value that the packets start with, $\mathcal M_{TTL}$, is not too small (compared with the number of hops before the loop $B$, the loop length $L$, and our parameter $T$) we have a decent probability of identifying the loop. Specifically, notice that if the first hop number at which $c$ became non-zero was at $\mathcal M_{TTL} - L\cdot T$, then the packet would complete another $T$ cycles over the loop and report it without being dropped. 
Therefore, we wish to lower bound the probability that $c$ is incremented during the first $\mathcal T-T$ cycles of the loop. Let $E_j$ denote the event that a successful detection started on the $j$'th cycle. That is, some hop on the $j$'th cycle sampled the packet, and no hop among the next $L$ changed the digest. We introduce an additional auxiliary variable $Q_\ell$ which denotes the event that a successful identification starts at the $\ell$'th hop.
We have that $\Pr[Q_\ell]=1/\ell \cdot \prod_{q=\ell+1}^{\ell+L}(q-1)/q = 1/(\ell+L)$ and thus
\begin{multline*}
    \Pr[E_j] = \sum_{\ell=B+(j-1)L+1}^{B+jL} Q_\ell = H_{B+jL}-H_{B+(j-1)L}\\
    \approx \ln\parentheses{\frac{B+jL}{B+(j-1)L}} = \ln\parentheses{1+\frac{L}{B+(j-1)L}}.
\end{multline*}

Next, we note that $\Pr[E_j\mid \neg E_{j-1}]\ge \Pr[E_j]$; that is, the probability of a successful identification in the $j$'th cycle increases when the $j-1$'th cycle did not identify the loop. Intuitively, either there was no hop that sampled the packet during the $j-1$'th cycle (at which case the probability for $E_j$ is not affected), or some hop has sampled it, but another has changed the digest before the packet completed a cycle. 
Finally, we have that 
\begin{multline*}
    \Pr[\mbox{detecting the loop}] \\= 1-\Pr[\neg E_1]\cdot \Pr[\neg E_2 \mid \neg E_1]\cdot \Pr[\neg E_3 \mid \neg E_2]\ldots\\
    \le 1-\prod_{\ell=1}^{\mathcal T-T}(1-\Pr[E_\ell])\le 1-\prod_{j=1}^{\mathcal T-T} \left(1-\ln\left(1+\frac{L}{B+jL}\right)\right).
\end{multline*}





==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#
# $Id: 
#

.SUFFIXES:
.SUFFIXES: .ps .dvi .tex

TEXINPUTS := .:${TEXINPUTS}
BIBINPUTS := .:${TEXINPUTS}

PDFLATEX ?= pdflatex
TEX = $(wildcard *.tex)

pdf: main.pdf

clean:
	$(RM) *.out *.aux *.thm *.log *.bbl *.blg *~ \#*\# *.toc *.idx
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

distclean: clean
	$(RM) $(patsubst %.fig, %.eps, $(wildcard *.fig))
	$(RM) $(patsubst %.obj, %.eps, $(wildcard *.obj))

%.pdf: $(TEX) $(wildcard *.bib)
	$(PDFLATEX) $*
	-bibtex $*
	if [ -e $*.toc ] ; then $(PDFLATEX) $* ; fi
	if [ -e $*.bbl ] ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	if egrep Rerun $*.log ; then $(PDFLATEX) $* ; fi
	$(PDFLATEX) $*


toc: $(wildcard *.tex)
	@egrep -h "\\\((sub)*section|chapter)" $+ | egrep -v "^%" | \
                sed -e 's/\\chapter//;                          \
                s/\\section/    /;                              \
                s/\\subsection/         /;                      \
                s/\\subsubsection/                      /;      \
                s/\\.*{//g;s/[{}]//g' > $@


==> graphs/Makefile <==
GNUPLOT ?= gnuplot

scripts := $(wildcard scripts/*.gpl)

.PHONY: graphs
graphs:
	for s in $(scripts); do \
	  $(GNUPLOT) $$s;\
	done

.PHONY: clean
clean:
	$(RM) *.pdf *.eps


==> relatedWorkTable.tex <==
\begin{table*}[]
\begin{center}
\resizebox{.5\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{c|c|c}
\hline
\multirow{ 2}{*}{\textbf{Solution}}             & \textbf{Per-packet}  		& \textbf{Topology}\\ 
						& \textbf{overhead}		& \textbf{dependancy}\\ \hline
\hline
\multirow{ 2}{*}{Path Queries~\cite{narayana16}}& depends on topology     	& \multirow{ 2}{*}{no}\\
                                                & size (order of bits)          & \\ \hline
\multirow{ 2}{*}{INT~\cite{int}}                & depends on topology     	& \multirow{ 2}{*}{no}\\
                                                & size (order of bytes)         & \\ \hline
\multirow{ 2}{*}{TPP~\cite{jeyakumar14}}        & depends on topology     	& \multirow{ 2}{*}{no}\\
                                                & size (order of bytes)         & \\ \hline
PathDump~\cite{tammana16}                       & up to 8B                      & small diameter \\\hline
IP Traceback~\cite{savage00}                    & 16 bits                       & no \\ \hline
\end{tabular}
}
\end{center}
\caption{State-on-packet solutions: overheads network topology dependancy}
\label{tab:state-on-pkt}
\end{table*}
\begin{table*}[]
\begin{center}
\resizebox{1.\textwidth}{!}{% <------ Don't forget this %
\begin{tabular}{c|l}
\hline
\textbf{Packet/info Mirroring} & \textbf{Description} \\ \hline
\hline
Everflow~\cite{zhu15} 			& Match and mirror on switch. From MS current deployment, the mirrored traffic volume	\\ 
					& is only 0.38\%. Given 100 Tbps of DCN traffic, the mirrored traffic requires 380 Gbps \\
					& network bandwidth and 300M pps CPU processing power. By default, they configure rules \\ 
					& in the TCAM table to match on TCP SYN/FIN/RST flags and n bits in the IPID field to   \\
					& sample 1 out of $2^n$ packets. For example, by configuring a rule to match on 10 bits \\
					& in the IPID field, they will sample 1 out of 1,024 packets.\\
Stroboscope~\cite{tilmans18}		& Query-based mirroring. From high-level queries, it automatically derives how to mirror \\
					& traffic so as to maximize monitoring accuracy without exceeding a budget. Example of 	\\
					& budget: USING 15 Mb/s DURING 450 ms EVERY 5 s. By coordinating packet mirroring across \\
					& routers, Stroboscope implements deterministic packet sampling: it collects copies of the \\
					& same packets from multiple locations, following such packets as they cross the network.\\
Planck~\cite{rasley14}			& Trace as much as they can. No query. In multiple (or all) ports are mirrored to a single \\ 
					& monitoring port, which introduces a problem: the total traffic flowing through the switch, \\
					& and thus mirrored to the monitoring port, often will exceed the capacity of the monitoring \\
					& port. When this happens, the switch mirrors as much as it can and drops the rest. They need \\
					& 275 microseconds to 4 milliseconds timescales on a 10 Gbps commodity to extract network information\\
NetSight~\cite{handigol14}		& They trace ALL packets header. They call it postcards. Problem discussed before on scalability\\
Trajectory Labels~\cite{duffield01}	& The key idea is to base the sampling decision on a deterministic hash function over the packet's\\ 
					& content. If the same hash function is used throughout the domain to sample packets, then a packet\\ 
					& is either sampled on every link it traverses, or on no link at all. To obtain trajectory samples,\\
					& it is then sufficient to obtain a unique packet identifier, or label, for each sampled packet (20bit)\\ 
\hline
\textbf{State-on-switch} & \textbf{Description} \\ \hline
\hline
Hash-based IP Traceback~\cite{snoeren01}& The router produces packet digests of each packet (32 bit), and stores the digests in a bloom filter.\\
                                        & Digest tables are stored locally at the router for some period of time, depending on the resource\\
                                        & constraints of the router. If interest is expressed in the traffic data for a particular time interval\\,
                                        & the tables are transferred to a collector. On router with 32 OC-192 links, the system would need 23.4GB\\
                                        & for one minute's worth of storage for the digest table.\\
FlowRadar~\cite{li16}         	& 2.88MB for 100K flows with 99\% decoding success (30MB for 1000K). It needs 2.3Gbps per switch to send encoded flowsets\\ 
					& of 100K flows with 10ms time slot. Decoding requires proportionally more cores with more switches.\\	
\hline
\textbf{State-on-packet} & \textbf{Description} \\ \hline
\hline
Path Queries~\cite{narayana16}          & Declarative path queries along with the network's forwarding policy, generating the switch-level rules\\ 
					& that process exactly the packets matching the queries, in operator-specified ways, e.g., counting, sampling\\ 
					& and mirroring. For 6 queries and a network topology of 16 routers, it needs 700 rules per switch and 16 bits\\ 
					& per packet. For bigger networks, 160 nodes, it would require 1400 rules and 32 bits per packet.\\
INT~\cite{int}				& to simply store the switch ID to be used in the path reconstruction, you need 4B each hop.  In addition you\\
					& also have 8B INT header. You need the packet to reach an end system to perform analysis = it suffers routing\\
					& loops. With INT header and space for 10 hops, this is 48 bytes/packet. If the average packet size is 1000 bytes,\\
					& this is a 4.8\% bandwidth overhead.\\
TPP~\cite{jeyakumar14}			& Similar to INT. The instruction overhead is 12 bytes/packet and 2 bytes of per-hop data to store the switchID.\\
					& With a TPP header and space for 10 hops, this is 32 bytes. If the average packet size is 1000 bytes, this\\
					& is a 3.2\% bandwidth overhead.\\
PathDump~\cite{tammana16}		& To trace packet trajectory selected switches (according to CherryPick) embeds its switchID. It only works\\
					& for small diameter networks. It requires up to 8B of packet data and also needs about 110 MB of disk space \\
					& to store 240K flow entries.\\
IP Traceback~\cite{savage00}		& requires 16 bits of packet header. It needs between 500 and 3000 packets to reconstruct a path from 1 hop to\\
					& 31 hops.\\
\end{tabular}
}
\end{center}
\caption{Related Work for Path Reconstruction.}
\label{tab:apps}
\end{table*}



